Counterfactual Variable Control for Robust and Interpretable Question Answering

Deep neural network based question answering (QA) models are neither robust nor explainable in many cases. For example, a multiple-choice QA model, tested without any input of question, is surprisingly "capable" to predict the most of correct options. In this paper, we inspect such spurious "capability" of QA models using causal inference. We find the crux is the shortcut correlation, e.g., unrobust word alignment between passage and options learned by the models. We propose a novel approach called Counterfactual Variable Control (CVC) that explicitly mitigates any shortcut correlation and preserves the comprehensive reasoning for robust QA. Specifically, we leverage multi-branch architecture that allows us to disentangle robust and shortcut correlations in the training process of QA. We then conduct two novel CVC inference methods (on trained models) to capture the effect of comprehensive reasoning as the final prediction. For evaluation, we conduct extensive experiments using two BERT backbones on both multi-choice and span-extraction QA benchmarks. The results show that our CVC achieves high robustness against a variety of adversarial attacks in QA while maintaining good interpretation ability.

==> sections/7_broader_impact.tex <==
% \section*{The Potential Broader Impact}
\section*{Broader Impact}

We believe that this work has potential positive societal impact in at least the following two ways: 
(1) Our work addresses the robustness issue in Question Answering.
Question Answering systems can potentially be applied to a wide range of application domains. 
For example, many chatbot systems providing customer services are essentially FAQ systems, so they employ QA techniques to locate answers from large text corpora to questions raised by customers.
In healthcare, QA systems can help patients to seek healthcare-related information more easily before or even without consulting a doctor.
QA systems can also assist general knowledge sharing, such as to assist users of platformas such as Stack Exchange and Quora to quickly find relevant answers to their questions.
% In the education domain, question answering system (model) is able to generate the answer for specific question and assist teacher in learning~\cite{atapattu2015educational}. 
% In healthcare caring, patients are able to seek health care information via question answering. In industry domain, Question Answering also plays important role in e-Commerce, social media, etc.
(2) Our technique for improving the robustness of QA is general and can be potentially applied to deep learning based models for other tasks as well to improve their robustness.
Improving the robustness and interpretability of deep learning models has significant implications beyond just increasing model accuracy.
For example, in our paper we showed that our techniques can be used to make QA models less vulnerable to adversarial examples compared with standard models.
This could prevent QA systems from malicious attacks.
Building interpretable models is also crucial for building the trust by humans in machine learning systems, which has attracted much attention in the research community in recent years.

% Although the performance of deep learning models have been improving, there is always a problem that the models are lack of robustness interpretability~\cite{lipton2018mythos,carlini2017towards}.
% From the aspect of robustness, the models are vulnerable to adversarial attacks, \eg, adding one question mark to the question may completely change the prediction of Question Answering model. More seriously, by adjusting the input passage one can manipulate the output to specific offensive words~\cite{wallace2019universal}.
% From the aspect of interpretability, we humans not only want the good performance but also expect the model to be interpretable when we are going to deploy it. 
Therefore, we believe that by focusing on both robustness and interpretability of deep learing based Question Answering models, our work has a significant broader impact.
% one concerns of applying deep learning model is that most of them are lack of interpretability and vulnerable to adversarial attacks~\cite{lipton2018mythos,carlini2017towards}. It makes
% Our work also aims to fill this blank.
% Our work
% our work aims to provide robustness and interpretability which humans are mainly concerned recently~\cite{lipton2018mythos,carlini2017towards}.
% (3)

==> tables/data_aug.tex <==
\begin{table}[]
    \centering
    \footnotesize
    \setlength\tabcolsep{2pt}
    \begin{tabular}{llllllllllll}
\toprule 
                                              &          & \texttt{Test} & \texttt{Adv1} & \texttt{Adv2} & \texttt{Adv3} & \texttt{Adv4} & A.G. \\\midrule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Add Adv1}}} & CT       & 71.0 & 70.6 & 72.1 & 42.5 & 60.5 & - \\
\multicolumn{1}{c}{}                          & CVC-IV    & 71.7 & 73.3 & 74.9 & 49.2 & 63.8 & +3.9\% \\\midrule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Add Adv2}}} & CT       & 72.3 & 73.0 & 75.1 & 50.1 & 63.3 & - \\
\multicolumn{1}{c}{}                          & CVC-MV & 71.8 & 74.2 & 76.6 & 61.1 & 65.5 & +3.9\% \\\midrule
\multirow{2}{*}{\textbf{Add Adv3}}                     & CT       & 67.5 & 62.7 & 59.9 & 70.9 & 57.1 & - \\
                                              & CVC-IV    & 67.6 & 64.5 & 62.4 & 70.2 & 61.6 & +2.0\% \\\midrule
\multirow{2}{*}{\textbf{Add Adv4}}                     & CT       & 69.8 & 65.4 & 60.2 & 27.7 & 63.3 & - \\
                                              & CVC-IV    & 69.9 & 66.2 & 62.4 & 32.7 & 61.0 & +1.4\% \\\midrule
\multirow{3}{*}{\textbf{Add All}}                      & CT       & 70.5 & 72.1 & 74.1 & 72.5 & 63.4 & - \\
& CVC-IV & 72.7 & 73.5 & 76.4 & 71.9 & 68.4 & +2.0\% \\ 
                                              & CVC-MV & \textbf{73.1} & \textbf{74.6} & \textbf{76.6} & \textbf{73.3} & \textbf{73.5} & \textbf{+4.0\%}\\
\bottomrule  
\end{tabular}
\caption{[can be moved to supple] Accuracies(\%) of BERT-base
models trained with data augmentation on MCTest.}
% with different kinds of data augmentation in training with BERT-base.}
\label{augment}
\end{table}

==> tables/data_aug_part.tex <==
\begin{wraptable}{r}{9cm}
\centering
\setlength\tabcolsep{3pt}
\footnotesize
\vspace{-0.65cm}
\caption{Accuracy(\%) on MCTest dataset with different kinds of data augmentation in training with BERT-base. Only the results of better performed method are shown here.}
\begin{tabular}{llllllllllll}
\toprule 
                                              &          & Test & Adv1 & Adv2 & Adv3 & Adv4 & AG \\\midrule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Add Adv1}}} & CT       & 71.0 & 70.6 & 72.1 & 42.5 & 60.5 & - \\
\multicolumn{1}{c}{}                          & CVC-IV    & 71.7 & 73.3 & 74.9 & 49.2 & 63.8 & +3.9\% \\\midrule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Add Adv2}}} & CT       & 72.3 & 73.0 & 75.1 & 50.1 & 63.3 & - \\
\multicolumn{1}{c}{}                          & CVC-MV & 71.8 & 74.2 & 76.6 & 61.1 & 65.5 & +3.9\% \\\midrule
\multirow{2}{*}{\textbf{Add Adv3}}                     & CT       & 67.5 & 62.7 & 59.9 & 70.9 & 57.1 & - \\
                                              & CVC-IV    & 67.6 & 64.5 & 62.4 & 70.2 & 61.6 & +2.0\% \\\midrule
\multirow{2}{*}{\textbf{Add Adv4}}                     & CT       & 69.8 & 65.4 & 60.2 & 27.7 & 63.3 & - \\
                                              & CVC-IV    & 69.9 & 66.2 & 62.4 & 32.7 & 61.0 & +1.4\% \\\midrule
\multirow{2}{*}{\textbf{Add All}}                      & CT       & 70.5 & 72.1 & 74.1 & 72.5 & 63.4 & - \\
                                              & CVC-MV & \textbf{73.1} & \textbf{74.6} & \textbf{76.6} & \textbf{73.3} & \textbf{73.5} & \textbf{+4.0\%}\\
\bottomrule  
\label{data_aug_part}
\end{tabular}
\vspace{-1cm}
\end{wraptable}

==> tables/ref_.tex <==
\begin{minipage}{\textwidth}
        \begin{minipage}[t]{0.47\textwidth}
            \centering
            \makeatletter\def\@captype{table}\makeatother\caption{xxxx 111}
            \label{sup}
            \scalebox{0.72}{
            \begin{tabular}{lccccc}
    \toprule
    \multirow{2}{*}{Methods} &
    \multicolumn{2}{c}{Market} &&
    \multicolumn{2}{c}{Duke} &

    \cline{2-3} \cline{5-6} 
    & mAP  & Rank-1   && mAP & Rank-1   \\
    \midrule
    %AlignedReID++ \cite{luo2019alignedreid++} & 77.6 & 91.0  && 68.0 & 80.7 \\
    FD-GAN'18 \cite{ge2018fd}  & 77.7   & 90.5    && 64.5 & 80.0   \\
    VPM'19 \cite{sun2019perceive}  & 80.8 & 93.0    && 72.6 & 94.2    \\
    PCB-RPP'18 \cite{sun2018beyond}  & 81.6 & 93.8   && 69.2 & 83.3  \\
    Mancs'18 \cite{wang2018mancs} & 82.3 & 93.1   && 71.8 & 84.9  \\
    HPM'19 \cite{fu2019horizontal}  & 82.7 & 94.2  && 74.3 & 86.6   \\
    CASN(PCB)'19 \cite{zheng2019re}  & 82.8 & 94.4  && 73.7 & 87.7  \\
    IANet'19 \cite{hou2019interaction} & 83.1 & 94.4  && 73.4 & 87.1   \\
    AANet'19 \cite{tay2019aanet}  & 83.4 & 93.9   && 74.3 & 87.7 \\
    CAMA'19 \cite{yang2019towards}  & 84.5 & 94.7  && 72.9 & 85.8  \\    
    DG-Net'19 \cite{zheng2019joint}  & 86.0 & 94.8   && 74.8 & 86.6 \\
    st-ReID'19 \cite{wang2019spatial}  & 86.7 & 97.2   && 82.8 & 94.0  \\
    MGN'18 \cite{wang2018learning}  & 86.9 & 95.7   && 78.4 & 88.7 \\
    DSA-reID'19 \cite{zhang2019densely}  & 87.6 & 95.7  && 74.3 & 86.2\\
    Pyramid'19 \cite{zheng2019pyramidal}  & 88.2 & 95.7   && 79.0 & 89.0  \\
    ABD-Net'19 \cite{chen2019abd}  & \textbf{88.3} & 95.6   && 78.6 & 89.0  \\
    \bottomrule
  \end{tabular}}
        \end{minipage}
        \hspace{0.03\textwidth}
        \begin{minipage}[t]{0.47\textwidth}
        \centering
        \makeatletter\def\@captype{table}\makeatother\caption{xxxx 222}
        \label{da}
        \scalebox{0.72}{
             \begin{tabular}{llcccc}
    \toprule
    \multirow{2}{*}{Methods} &
    \multicolumn{2}{c}{Market-to-Duke} &&
    \multicolumn{2}{c}{Duke-to-Market} &
    \cline{2-3}\cline{5-6}
    & mAP  & Rank-1   && mAP & Rank-1  \\
    \midrule
    PUL'18 \cite{fan2018unsupervised} & 16.4 & 30.0  && 20.5 & 45.5 \\
    TJ-AIDL'18 \cite{wang2018transferable}  & 23.0   & 44.3    && 26.5 & 58.2    \\
    SPGAN'18 \cite{deng2018image}  & 22.3 & 41.1   && 22.8 & 51.5    \\
    HHL'18 \cite{zhong2018generalizing}  & 27.2 & 46.9   && 31.4 & 62.2     \\
    CSFM'19 \cite{chang2019disjoint} & 27.3 & 49.8   && 28.3 & 61.2    \\
    BUC'19 \cite{lin2019bottom}  & 27.5 & 47.4   && 38.3 & 66.2   \\
    ARN'18 \cite{li2018adaptation}  & 33.4 & 60.2   && 39.4 & 70.3    \\
    UDAP'18 \cite{song2018unsupervised} & 49.0 & 68.4   && 53.7 & 75.8  \\
    ENC'19 \cite{zhong2019invariance}  & 40.4 & 63.3   && 43.0 & 75.1   \\
    UCDA-CCE'19 \cite{qi2019novel}  & 31.0 & 47.7   && 30.9 & 60.4 \\    
    PDA-Net'19 \cite{li2019cross}  & 45.1 & 63.2  && 47.6 & 75.2   \\
    SSG'19 \cite{fu2019self} & 53.4 &73.0 &&58.3 &80.0\\
    PCB-PAST'19 \cite{zhang2019self}  & 54.2 & 72.4   && 58.3 & 80.0   \\
    Co-teaching'18 \cite{han2018co}  & 55.7 & 71.9  && 65.1 & 82.5  \\
    MMT-700'20 \cite{ge2020mutual}  & 65.1 & 78.0   && 69.0 & 86.8  \\

    \bottomrule
  \end{tabular}}
        \end{minipage}
    \end{minipage}

==> tables/remove_part.tex <==
% \begin{table}[h]
% \caption{Accuracy of official test set under different inputs of four MCQA datasets trained with BERT-base.}
%   \label{table:remove_part_MCQA}
%   \centering
% \begin{tabular}{lllll}
% \toprule
% \multicolumn{1}{l}{}                     & \multicolumn{1}{l}{MCTest} & \multicolumn{1}{l}{DREAM} & \multicolumn{1}{l}{SemEval2018} & \multicolumn{1}{l}{RACE}  \\
% \midrule
% Random guess                               & 25.0                          & 33.3                       & 50.0                               & 25.0                         \\
% Full information                           & 68.9                       & 61.5                      & 87.5                            & 64.7                       \\
% No passage                                 & 24.2                       & 32.8                      & 69.7                            & 41.6                      \\
% No Question                                & 52.5                        & 57.1                      & 83.5                            & 51.0                      \\ 
%  \bottomrule
% \end{tabular}
% \end{table}



% \begin{table}[h]
% \centering
% \begin{minipage}{.6\linewidth}
% \centering
% \caption{Accuracy of official test set under incomplete inputs of three MCQA datasets trained with BERT-base.\yu{These two table move to supplementary?}\qianru{can be merged into one table: e.g. left region is MC, right is SQ}}
% \label{table:remove_part_MCQA}
% \begin{tabular}{lllll}
% % \caption{Accuracy of official test set under different inputs of four MCQA datasets trained with BERT-base.}
% % \label{table:remove_part_MCQA}
% \toprule
% \multicolumn{1}{l}{}                     & \multicolumn{1}{l}{MCTest} & \multicolumn{1}{l}{DREAM} &  \multicolumn{1}{l}{RACE}  \\
% \midrule
% Random guess                               & 25.0                          & 33.3                                                    & 25.0                         \\
% Full information                           & 68.9                       & 61.5                           & 64.7                       \\
% No \textit{P}                                 & 24.2                       & 32.8                           & 41.6                      \\
% No \textit{Q}                                & 52.5                        & 57.1                            & 51.0                      \\ No \textit{P} \& no \textit{Q}
%       &22.4
%       &33.4
%       &34.7                                \\
%  \bottomrule
% \end{tabular}
% \end{minipage}
% \hspace{0.5cm}
% \begin{minipage}{.3\linewidth}
% \centering
% \caption{F1 score of official dev set on SQuAD under incomplete inputs, the model is trained with BERT-base.}
% \label{table:remove_part_SEQA}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{ll}
% \toprule
%             & SQuAD   \\ \midrule
% Full information & 88.1 \\ 
% No \textit{N}   & 59.4 \\
% No \textit{V}   &55.1 \\
% No \textit{N} \& no \textit{V}  &15.3 \\
% No \textit{Q}   &12.4  \\
% \bottomrule
% \end{tabular}}
% \end{minipage}
% \end{table}

\begin{wraptable}
\centering
\scriptsize
\setlength\tabcolsep{3pt}
\caption{Accuracy of MCQA task (left side of table) and F1 score of SEQA task(right side of table) under incomplete inputs. The models are trained by full information with BERT-base. `RG' means random guess.}
\vspace{1pt}
\begin{tabular}{llll||ll}
\toprule
                 & MCTest & DREAM & RACE &                  & SQuAD \\ \midrule
RG     & 25.0   & 33.3  & 25.0 & Full & 88.1  \\
Full & 68.9   & 61.5  & 64.7 & No N             & 59.4  \\
No \textit{P}             & 24.2   & 32.8  & 41.6 & No \textit{V}             & 55.1  \\
No \textit{Q}             & 52.5   & 57.1  & 51.0 & No \textit{N}, \textit{V}     & 15.3  \\
No \textit{P}, \textit{Q}     & 22.4   & 33.4  & 34.7 & No \textit{Q}             & 12.4 \\\bottomrule
\end{tabular}
% \label{table:remove_part}
\end{wraptable}
